Icebergs in the Clouds: the Other Risks of Cloud Computing

Cloud computing is appealing from management and efficiency perspectives, but brings risks both known and unknown. Well-known and hotly-debated information security risks, due to software vulnerabilities, insider attacks, and side-channels for example, may be only the "tip of the iceberg." As diverse, independently developed cloud services share ever more fluidly and aggressively multiplexed hardware resource pools, unpredictable interactions between load-balancing and other reactive mechanisms could lead to dynamic instabilities or "meltdowns." Non-transparent layering structures, where alternative cloud services may appear independent but share deep, hidden resource dependencies, may create unexpected and potentially catastrophic failure correlations, reminiscent of financial industry crashes. Finally, cloud computing exacerbates already-difficult digital preservation challenges, because only the provider of a cloud-based application or service can archive a "live," functional copy of a cloud artifact and its data for long-term cultural preservation. This paper explores these largely unrecognized risks, making the case that we should study them before our socioeconomic fabric becomes inextricably dependent on a convenient but potentially unstable computing model.

==> preserv.tex <==
\section{Digital Preservation of Cloud-Based Artifacts}
\label{sec-preserv}

Again for space reasons,
this proposal merely sketches one preliminary approach
to addressing the problem of preserving cloud-based digital artifacts,
discussed in Section~\ref{sec-motiv-preserv}.
Two major factors make preservation difficult for cloud artifacts:
an incentive factor and a size factor.
We discuss and address each in turn.

The incentive problem is that in a cloud-based computing model,
the application or service provider need not, and has little incentive to,
make publicly available all the software and data underlying the service
that would be necessary for accurate historical preservation.
Competitiveness considerations, in fact,
offer the provider considerable incentive {\em not} to make available
the ``secret sauce'' underlying their products, in any form.
This incentive has long led traditional software vendors
to release their software only in binary form---%
often with deliberate obfuscation to thwart analysis---%
but only the cloud model frees the vendor entirely
from the need to release their code in {\em any} form
directly executable by the customer.
This incentive problem is probably unsolvable
by technical means alone:
we may have to institute
social, commercial, and/or governmental incentives
for providers to make their cloud-based artifacts preservable.
One first step might be for a major potential purchaser
of cloud-based services---%
the US government, for example---%
to demand purchased services to meet some archivability criterion,
much as the government already drives the development and deployment
of many security standards such as SHA and AES.

Assuming the proper incentives can be established,
the more technical part of the problem is that
cloud-based services often rely on enormous, frequently-changing datasets,
such as the massive distributed databases underlying Google Search or Maps
or an MMOG's virtual world.
It would probably be impractically costly for providers
to ship regular snapshots of their entire datasets to digital archivists---%
even well-provisioned ones such as the Library of Congress---%
not to mention impractically costly for the receiving archivists
to do anything with such enormous snapshots beyond saving the raw bits
in the hope they might become useful (and manageable) sometime in the future.

An approach more likely to be practical takes advantages of two observations.
First, in the short term,
it is much more efficient---%
hence much more likely to be technically and economically feasible---%
for archival snapshots of the provider's datasets
to remain largely resident on the same storage infrastructure
holding the ``live,'' master datasets from which these snapshots are taken.
Standard copy-on-write cloning and deduplication technologies~\cite{
	santry99elephant,quinlan02venti}
offer building blocks for maintaining such snapshots efficiently.
The more significant challenge may be
{\em protecting} and {\em administering}
these archival snapshots appropriately.
Archivists will desire strong guarantees
that historical snapshots will not be accidentally lost or deleted,
or maliciously tampered with by rogue provider employees,
while held on the provider's infrastructure.
Techniques currently being explored to protect a user's information privacy
from a host cloud provider~\cite{gu11certikos,zhang11cloudvisor}
may be adaptable to this purpose.
Further, since it is primarily the service's customers, and not the provider,
who wish for these snapshots to be stored,
the storage infrastructure should be able to account for
and ``charge'' appropriately
the relevant storage costs,
sharing them proportionately among the (potentially many) stakeholders
wishing for the provider's service to be historically preserved.
Ideally, using virtualization and shadowing technologies~\cite{
	dunlap02revirt,alimi08shadow},
historical snapshots of the cloud service should remain ``runnable''
and dynamically usable by all stakeholders in the snapshots:
e.g., a customer or historian could use the provider's infrastructure
to run a new Web search query
on a working copy of the search engine and its database
as they existed at a particular historical moment.

The second observation is that in the longer term,
the raw cost of safely {\em storing} historical snapshots
is likely to decrease rapidly with the age of the stored data,
as the density and cost-efficiency of mass storage continues to explode---%
while the difficulty and potential costs
of making snapshots {\em usable} is likely to increase with age,
as the original hardware and OS infrastructure that hosted the cloud server
becomes obsolete and is replaced with newer,
not-quite-compatible hardware and operating systems.
While it may be too costly to transfer and store complete snapshots
of a cloud service's state off the provider's own physical infrastructure
immediately after the snapshot is taken,
after 10 years for example,
the intervening increases in readily-available network and storage capacity
may make it practical to transfer and store complete 10-year-old snapshots
off the provider's infrastructure (e.g., at long-term digital libraries).

The PI has already done work towards addressing
the latter issue of maintaining the usability of archived software.
VXA~\cite{ford05vxa,ford08vx32} is an archival storage system that uses
lightweight virtualization and sandboxing techniques
to create OS-independent ``executable archives''
that may be more amenable to long-term preservation
than conventional software.
This and other emulation-based preservation techniques~\cite{
	rothenberg99avoiding,lorie00archiving,lorie02uvc}
are merely a start, however,
and will require substantial adaptation to the large-scale cloud context.



==> tifc.tex <==
\section{Timing Information Flow Control}
\label{sec-tifc}

This section introduces
a model for controlling an application's perception of time,
which we call {\em Timing Information Flow Control} or TIFC.
TIFC is inspired by recent work in
Decentralized Information Flow Control (DIFC)~\cite{
        efstathopoulos05labels,zeldovich06making,krohn07information},
but serves the purpose of controlling the propagation of
{\em information about time} into, out of, or within a software system.
With TIFC,
an operating system can attach explicit labels or {\em taints}
to processes and other objects,
describing what sources, types, and granularities of timing information
may have affected the state of the labeled object.
Using these labels,
the OS can enforce policies constraining
how timing-derived information may flow among processes
and affect their results.

\com{
(from NSF Det proposal...)

While many organizations see strong economic or practical motivations
to move compute-intensive applications
onto shared clusters or cloud services such as EC2~\cite{amazon-ec2},
sharing can create considerable information security and privacy concerns.
Even if the cloud provider itself is trustworthy
and its virtualization software correctly prevents
clients from directly interfering with each other,
any client's software can mount a variety of timing attacks
on other client processes running on the same or nearby hosts
to steal valuable secrets~\cite{brumley03remote,percival05cache},
provided the attacking process has fine-grained timing capability.
But many compute-bound applications suited to cloud computing
have no inherent need for fine-grained timing:
most data analysis applications merely compute a result
from a well-defined input dataset.
If a provider offered a compute cloud
in which no client has fine-grained timing capability,
the only timing information with which one client could attack another
would be the much coarser and noisier total job completion times
observed from the clients' own hosts.
A provider cannot create such a ``timing channel-free'' compute cloud
merely by disabling client access to hardware clocks and timers,
however:
an attacker's hosted code could use many other sources of nondeterminism
to regain fine-grained timing capability,
such as by spawning a thread that counts iterations of a spin-loop.
Only fully timing-insensitive execution
can guarantee a shared environment free of timing attack channels.


(from CRASH proposal...)

The second unique aspect of our kernel design is that it will address
not just conventional, explicit interactions between processes,
but also covert timing channels~\cite{kemmerer83shared,wray91analysis},
which have been largely avoided in previous IFC work
but are becoming increasingly critical to real-world security~\cite{
	brumley03remote,percival05cache,wang06covert,
	aciicmez07predicting,aciicmez07yet,ristenpart09cloud}.
Further leveraging our work in deterministic execution
and combining them with classic IFC techniques,
we will design the kernel to provide pervasive controls over
how and when potentially sensitive timing information
can enter or affect the results of
any untrusted application computation.
We describe these ideas in more detail elsewhere~\cite{ford10determinating}.

If we wish to timeshare a CPU core between two untrusted processes
and prevent timing channels between them, for example,
a classic approach would be to arrange a fixed timeslice for each process,
not varying depending on either process's actual usage,
and clear all caches and other state affecting timings on context switches.
While this approach may be useful in some situations,
it is undesirable due to the potential waste of resources it incurs,
due to the flushing of potentially useful state
and giving up the ability of one process to utilize fully
any resources left underutilized by others.
An alternative solution we will explore is to
timeshare the processes without restriction,
but run them deterministically
and thus prevent them from being able to ``tell the time'' locally
while running on the timeshared CPU core.
If one process has a semantic need to tell the time,
its ``read time'' request leads to an IFC ``taint'' fault,
e.g., causing the process to be migrated to some other CPU core
that is not timeshared at fine granularity between untrusted processes,
and on which the system time is thus ``untainted''
by information from other processes.

Taking this approach further,
suppose a process wishes to run on timeshared cores for performance,
but also use fine-grained internal timers
to make decisions for load-balancing parallel computations across cores
or similar internal optimization purposes.
In this case, instead of reading ``tainted'' high-resolution timers directly,
the process can fork off a parallel process
to make dynamic load-balancing decisions on behalf of the original process.
This new load-balancing process will become tainted
by timing information from other processes sharing the same core.
The kernel's determinism and IFC enforcement mechanisms, however,
will allow the tainted process to affect only the {\em scheduling}
(and hence execution performance) of the original process it was forked from,
and not the actual {\em results} computed by that process;
the original process will thus run (deterministically)
without itself becoming tainted with potentially leaked timing information.
}%xxx

To create a preliminary TIFC model,
we choose to build on the DIFC model used in Flume~\cite{
        krohn07information}
due to its simplicity and elegance.
Comparable TIFC models could probably be built ``stand-alone''
or as extensions to other DIFC systems, however.
Like Flume, our model
uses {\em tags} and {\em labels} to track information
as it flows through a system---%
potentially any type of information,
but here we focus exclusively on timing information.

\subsection{TIFC Model Overview}

As in Flume,
our TIFC model assigns {\em labels} to information-bearing system objects
such as processes, messages, and files.
A label can contain any number of {\em tags},
each if which indicates that the labelled object has a particular ``taint,''
or may be derived from information owned by a particular user.
Unlike conventional DIFC, however,
TIFC labels reflect not only the {\em content} contained in such an object---%
i.e., the information contained in the bits
comprising a message or a process's state---%
but also information that may have effected the timing
of observable {\em events} associated with that object---%
a process starting or stopping, a message being sent or received, etc.
Consistent with conventional, informal practices
for reasoning about timing channels~\cite{kemmerer83shared,wray91analysis},
our TIFC model does not attempt the likely-infeasible task
of eliminating timing channels entirely,
but rather seeks to impose strong limits on the {\em rate}
at which information might leak via timing channels.

To distinguish content and timing taint explicitly,
we give TIFC labels the form $\{L_C/L_T\}$,
where $L_C$ is a set of tags representing content taint,
and $L_T$ is a set of tags representing timing taint.
As in Flume, content tags in the set $L_C$
simply identify a user, such as Alice or Bob.
Timing tags, however, we give the form $P_f$,
where $U$ is a user such as Alice or Bob,
and $f$ is a frequency representing the maximum rate
with which user $U$'s information might leak via this timing event,
in bits per second.
The frequency part of a timing tag may be $\infty$,
indicating that information leakage may occur at an unbounded rate.
Thus, the label $\{A/A_\infty,B_f\}$ attached to a message
might indicate that the content (bits) comprising the message
contains Alice's (and only Alice's) information,
but that the {\em timing} with which the message was sent
might contain (and hence leak) both Alice's and Bob's information---%
at an arbitrarily high rate in Alice's case,
but up to at most $f$ bits per second in Bob's case.

\subsubsection{Declassification Capabilities}

To enforce information security policies,
we similarly build on Flume's DIFC model.
In particular,
the system allows a given process $P$ to transmit information
to another process or target object $O$
only if $P$'s label is a subset of $O$'s,
or if $P$ holds {\em declassification capabilities}
for any tags in $P$ that are not in $O$.
A {\em content declassification capability} has the form $U^-$,
and represents the ability to remove content tag $U$,
as in Flume.
TIFC also adds {\em timing declassification capabilities}
of the form $U^-_f$,
representing the ability to declassify information
carried by timing channels at a rate up to frequency $f$.
We consider the ``maximum-strength'' timing declassifier
$U^-_\infty$ to be equivalent
to the content declassifier $U^-$;
other timing capabilities with finite frequencies
represent weakened versions of these infinite-rate capabilities.

Suppose process $P_1$ has label $\{A/A_\infty,B_f\}$,
and process $P_2$ has the empty label $\{-/-\}$.
If process $P_1$ were allowed to send a message to $P_2$,
this action would leak $A$'s information via both message content
and the timing of the message's transmission,
and would leak $B$'s information (at a rate up to $f$)
via timing alone.
The system will disallow this communication, therefore,
unless the processes hold and use the relevant capabilities
to adjust their labels before interacting.
In particular:
(a) $P_1$ must hold the capability $A^-$
and use it to remove its content tag $A$ before sending the message; and
(b) $P_1$ must hold and use a timing capability $B^-_f$ (or stronger) 
to declassify timing tag $B_f$ before sending the message.

\subsection{Controlling Timing Channels with Determinism and Pacing}

Timing labels and capabilities alone would not be very useful
without practical mechanisms to control the timing information flows
they represent.
We briefly introduce two specific tools useful for this purpose:
{\em deterministic execution} and {\em pacing}.
This section briefly describes these tools,
and the next section illustrates how we may be able to use them
to control timing channels in practical systems.

\paragraph{Deterministic Execution:}

In general, a process whose label contains content tag $U$
must also have timing tag $U_\infty$,
because the process's flow of control---and hence execution time---%
can vary depending on the $U$-owned bits contained in its process state.
(We could envision special-purpose ``data-invariant''
execution models or processors that avoid flow control
and guarantee the same execution time on any input,
but such processors would be of limited use and are not our focus.)
It might also seem that the converse should be true:
if a process has timing tag $U_f$ for any frequency $f$,
and the process reads the current time via \verb|gettimeofday()|, for example,
then the process's content subsequently depends on its prior execution timing,
hence the process would have to be given content tag $U$.
Even if we disable system calls like \verb|gettimeofday()|,
conventional programming models---especially parallel, multithreaded models---%
offer innumerable ways in which processes and threads
can observe and depend on their execution timing in implicit ways,
such as by measuring the relative execution speed of different threads.
For example,
one thread might simply remain in a tight loop 
forever incrementing a counter in shared memory,
which other threads read and use as a ``timer.''

The PI's recent work in 
system-enforced deterministic parallel execution~\cite{
	ford10efficient},
however,
offers a new tool to decouple a process's timing and content labels.
With system-enforced determinism,
as implemented in the PI's Determinator OS,
the kernel can prevent unprivileged processes from exhibiting
{\em any} timing dependencies---%
even if the process maliciously attempts to introduce such dependencies---%
except via explicit inputs obtained through controlled channels.
In effect, deterministic processes cannot ``tell time''
except via timing information contained in their explicit inputs
controlled by their content labels.
With system-enforced deterministic execution, therefore,
it becomes ``safe'' for a process's content and timing labels to differ.
If a process's explicit inputs were derived from user $A$'s information,
but the timing of its execution
was also affected by $B$'s information at rate $f$,
we can give the process the label $\{A/A_\infty,B_f\}$
rather than $\{A,B/A_\infty,B_f\}$,
safe in the knowledge that system-enforced determinism
prevents $B$'s ``timing domain'' information
from leaking into the process's ``content domain''
(i.e., its register/memory state).

\paragraph{Pacing:}

Processes often interact with each other and with the external world
via queued messages or I/O requests,
and we can leverage ``traffic shaping'' techniques
common in the networking world
to limit the rate at which information might leak across these queues
via timing channels.
In particular,
we assume that we can {\em pace} the output of a message queue,
such that regardless of how messages build up in the queue,
the queue's output ``releases'' at most one message per tick
of some recurring timer firing at a given frequency $f$.
That is, after each $1/f$-time period,
the queue's output releases exactly one message if the queue is non-empty,
and no message if the queue is empty at that point.
Between clock ticks, the queue releases no information at all.
Ignoring any information contained
in the {\em content} and {\em order} of the queued messages---%
which we will control via content labels---%
we can see that such a paced queue leaks at most one bit of timing information
per $1/f$-time period:
namely, whether or not the queue was empty at that particular timer tick.
That is, if the messages flowing into a paced queue
have a timing tag of $U_f'$ for $f' > f$ (including $f' = \infty$),
then we can safely ``downgrade'' the timing tags of those messages to $U_f$
as they emerge from the queue,
if $f$ is the queue's pacing frequency.
If messages with label $\{A/A_\infty,B_\infty\}$
flow into a pacer with frequency $f$, for example,
for example,
then the messages emerging from the queue's output
have label $\{A/A_f,B_f\}$.
While we for now offer only an intuitive argument
for the correctness of this rate-limiting mechanism,
I believe this argument can be precisely formalized,
and intend to do so as part of the further development of the TIFC model.

\subsection{TIFC Examples}

Instead of delving into this preliminary TIFC model in more detail,
we merely illustrate its potential uses via three simple examples.
In these examples, two customers---%
Alice and Bob---%
each wish to perform some privacy-sensitive computation
on cloud hardware managed by a trusted cloud provider.
Each customer would like strong assurance from the provider
that his sensitive data cannot leak to other customers
beyond some well-defined rate---%
even if his code is infected with malware
that deliberately attempts to use timing channels to leak his data.
For these examples we make the simplifying assumption
that timing channels arise only from shared compute resources,
such as processor cores and the caches and functional units supporting them.
We neglect for now other sources of timing channels,
such as those arising from network communication paths
either within the cloud or between cloud and customers~\cite{
	ristenpart09cloud},
although this TIFC model should readily extend
to the handling of communication-related timing channels as well.

\paragraph{Dedicated Hardware Scenario:}

The first example,
in Figure~\ref{fig-private}(a),
illustrates a trivial ``base case'' scenario,
in which the cloud provider controls timing channels
merely by imposing a fixed partitioning of hardware compute resources
between Alice and Bob.
Alice submits compute job requests
via a cloud gateway node that the provider dedicates exclusively to Alice,
and similarly for Bob.
Each customer's gateway node forwards each submitted compute job
to some compute core (on the same or a different node)
that is also dedicated exclusively to the same customer.
The provider's trusted gateway nodes
attach TIFC labels to each incoming request,
and the provider's trusted OS kernel or hypervisor
managing each compute core
uses these labels to prevent either customer's compute jobs
from leaking information to the other
via either the content or timing of messages within the cloud.

Figure~\ref{fig-private}(b) and (c)
illustrates the (intuitively trivial) reason
this example provides timing isolation,
by contrasting the system's timing when Bob submits a ``short'' job (b)
with the timing when Bob submits a ``long'' job (c).
Since Alice's job runs on a separate compute core from Bob's,
Alice's job completion time depends only on
the content of that job and Alice's prior jobs---%
information represented by the timing tag $A_\infty$---%
and is not ``tainted'' by any timing dependency on Bob's jobs.

\begin{figure}[t]
\centering
\includegraphics[width=0.90\textwidth]{private.eps}
\caption{Content and Timing Information Labels:
	Private Per-Client Hardware Resources}
\label{fig-private}
\end{figure}

\paragraph{Fixed-Reservation Timeslicing Scenario:}

Figure~\ref{fig-reserved}(a)
shows a similar but slightly less trivial example,
in which a shared compute core
processes both Alice's and Bob's jobs
on a ``fixed reservation'' schedule that does {\em not} depend
on either Alice's or Bob's {\em demand} for the shared core.
This example assumes that the shared compute core
maintains and isolates the state of each customer's job
using standard process or virtual machine mechanisms.
The scheduling of these per-customer processors
onto the shared compute core, however,
is controlled by a separate entity we call the {\em reservation scheduler}.
The scheduler conceptually runs on its own dedicated CPU hardware,
and sends a message to the shared compute core
at the beginning of each timeslice
indicating which customer's job should be run during that timeslice.
The code implementing the scheduling policy
need not be trusted for information flow control purposes,
as long as trusted code attaches and checks TIFC labels appropriately.
In particular, the scheduler and the messages it sends have
the empty label $\{-/-\}$,
which allows the scheduler's messages to affect
the timing of Alice's and Bob's labeled jobs running on the shared core,
without adding any new ``taint.''
With its empty label, however,
the reservation scheduler cannot {\em receive} any messages
from the shared core
that might depend on either the content or timing of the customers' jobs.
In particular, TIFC enforcement prevents the scheduler
from obtaining any feedback about whether either Alice's or Bob's processes
actually demand CPU time at any given moment,
forcing the scheduler to implement a ``demand-insensitive'' policy,
which isolates the timing of different customers' jobs sharing the core
at the cost of wasting shared core capacity when any customer's demand is low.
Figure~\ref{fig-reserved}(b) and (c)
shows execution schedules for the shared core
in the cases in which Bob's job is short or long, respectively,
illustrating why Alice's job completion time
depends only on Alice's information---%
hence the timing label of $A_\infty$---%
even though Bob's job may have executed on the same core
during different (demand-independent) timeslices.

\begin{figure}[t]
\centering
\includegraphics[width=0.90\textwidth]{reserved.eps}
\caption{Labeling Scenario: Shared Resource with Reservation-based Scheduling}
\label{fig-reserved}
\end{figure}

\paragraph{Demand-Sensitive Statistical Multiplexing Scenario:}

The above ``dedicated hardware'' and ``reservation scheduling'' scenarios
embody well-known timing channel control techniques~\cite{
	kemmerer83shared,wray91analysis},
to which TIFC merely adds an explicit, enforceable labeling model.
These standard timing channel control techniques unfortunately
undermine the cloud {\em business model},
however,
by limiting or eliminating the cloud provider's ability
to obtain efficiencies of scale
through oversubscription and statistical multiplexing
of hardware resources~\cite{ford10determinating}.
Figure~\ref{fig-statmux} illustrates a final scenario
that {\em does} allow statistical multiplexing,
at the cost of a controlled-rate timing information leak.

\begin{figure}[t]
\centering
\includegraphics[width=0.90\textwidth]{statmux.eps}
\caption{Labeling Scenario: Shared Resource with Demand-driven Scheduling}
\label{fig-statmux}
\end{figure}

As in the previous example,
this scenario includes a shared compute core
and a separate scheduler entity.
In this case, however,
instead of the empty (minimum) label,
we give the scheduler a ``high'' (maximum) label
containing all customers' content and timing taints.
This high label allows the scheduler to receive
demand information about the customers' jobs from the shared compute core,
and even to receive messages from customers' jobs themselves
containing explicit scheduling requests or ``hints.''
Since the scheduler's content label ($A,B$)
is higher than the content labels of either Alice's or Bob's jobs,
TIFC disallows the scheduler from sending messages
{\em to} Alice or Bob,
or otherwise affecting the {\em content} (process state) of their jobs.

The scheduler can send messages
to the shared compute core's trusted control logic, however,
which uses these messages only to determine
which customer's jobs run during a particular timeslice.
The shared core runs these jobs deterministically, however,
ensuring that regardless of how the scheduler runs them,
each job's result content depends only on that job's input content
and not on any aspect of the job's execution timing.
The scheduler's control messages therefore ``taint'' all jobs
with the timing tags---but {\em not} the content tags---%
of all customers.
The results of Alice's job, for example,
has the label $\{A/A_\infty,B_\infty\}$,
indicating that the result content contains only Alice's information
but the timing of the job's completion may also contain Bob's information.
Without additional measures,
this high timing label would prevent Alice's gateway
from sending Alice's job results back to Alice,
since the timing of these job completion messages
could leak Bob's information at an arbitrarily high rate.

To rate-limit this timing leak,
we assume that when requesting service from the cloud provider,
Alice and Bob agreed to allow timing information leaks
up to a specific rate $f$ fixed throughout this particular cloud.
To enforce this policy,
the cloud provider inserts a pacer on the path
of each customer's job results queue,
which releases the results of at most one queued job
at each frequency $f$ ``tick'' of some trusted provider-wide clock.
In addition, since all customers have agreed to allow
timing information leaks up to rate $f$,
each user's gateway node gives all other gateways
a timing declassification capability for rate $f$:
thus, Alice's and Bob's gateways can declassify each others' timing labels
up to rate $f$.
With this system design,
the TIFC rules allow Alice's job results to flow back to Alice
at a rate of up to $f$ jobs per second,
while leaking at most $f$ bits per second of Bob's information.

As in the previous scenarios,
Figure~\ref{fig-statmux}(b) and (c) compares two execution schedules
resulting from Bob's job being ``short'' and ``long,'' respectively.
Due to demand-sensitive multiplexing,
each job's completion time depends on the prior jobs of all users,
possibly embodying all users' information at an arbitrary rate.
Alice's output pacer, however,
delays the release of each job's results to a unique clock tick boundary,
``scrubbing'' this timing channel down to the frequency $f$
at which the gateways can declassify the timing labels.


